Rethinking the Starting Point: Collaborative Pre-Training for Federated Downstream Tasks

A few recent studies have demonstrated that leveraging centrally pre-trained models can offer advantageous initializations for federated learning (FL). However, existing pre-training methods do not generalize well when faced with an arbitrary set of downstream FL tasks. Specifically, they often (i) achieve limited average accuracy, particularly when there are unseen downstream labels, and (ii) result in significant accuracy variance, failing to provide a balanced performance across clients. To address these challenges, we propose CoPreFL, a collaborative/distributed pre-training approach which provides a robust initialization for downstream FL tasks. The key idea of CoPreFL is a model-agnostic meta-learning (MAML) procedure that tailors the global model to closely mimic heterogeneous and unseen FL scenarios, resulting in a pre-trained model that is rapidly adaptable to arbitrary FL tasks. Our MAML procedure incorporates performance variance into the meta-objective function, balancing performance across clients rather than solely optimizing for accuracy. Through extensive experiments, we demonstrate that CoPreFL obtains significant improvements in both average accuracy and variance across arbitrary downstream FL tasks with unseen/seen labels, compared with various pre-training baselines. We also show how CoPreFL is compatible with different well-known FL algorithms applied by the downstream tasks, enhancing performance in each case.

==> Tab/Alg_pretraining.tex <==
\begin{algorithm*}[t]
% \begin{algorithm}
\caption{{\system} Our Pre-training Method (Pre-training Phase)}
\label{alg:alg_pretrain}
\begin{algorithmic}[1]
\State \textbf{Input:} Server dataset $D^S$, Client dataset $D^C$ 
\State Split $D^C$ to $M$ clients based on IID or non-IID distribution, and select $m \in M$ participants.
\State Each participant $j \in m$ partitions their own dataset $D_j$ into support set $S_j$ and query set $Q_j$
\If {Sever's dataset is not considered}
\For {Each communication round $r = 1, 2, ..., R$}
\State Participants download global model $\phi^{r-1}$
\For {Each participant $j$ in parallel}
\State Initialize each local model $\phi_j$ with $\phi^{r-1}$
\State $\mathcal{L}_{S_j}(\phi)$ $\gets$ $\frac{1}{|S_j|}$ $\sum_{(x,y) \in S_j}{} \ell(f_\phi(x), y)$
\State $\phi_{j}$ $\gets$ $\phi^{r-1}$ - $\eta \nabla \mathcal{L}_{S_j}(\phi)$ \Comment{Local update using support set $S_j$}
\EndFor
% \State $\overline{\phi^r}$ $\gets$ $\sum_{j=1}^{m} \frac{|S_j|}{|S|} \phi_j$
\State $\overline{\phi^r}$ $\gets$ $\sum_{j=1}^{m} \mu_j \phi_j$ \Comment{Model aggregation; $\mu_j$ is the relative support set size}
\For {Each participant $j$ in parallel}
% \State Initialize each local model $\phi_j$ with $\overline{\phi^r}$
\State Participants download $\overline{\phi^r}$ for initialization and perform meta-updates
\State $\mathcal{L}_{Q_j}(\phi)$ $\gets$ $\frac{1}{|Q_j|}$ $\sum_{(x,y) \in Q_j}{} \ell(f_\phi(x), y)$ \Comment{Local meta-update using query set $Q_j$}
\EndFor
\State Overall meta-loss: $\mathcal{L}_{Q} = \sum_{j=1}^{m} \mathcal{L}_{Q_j}(\phi) $; standard deviation of meta-losses: $\sigma_Q$ 
\State Customized Loss: $\mathcal{L} = \gamma \mathcal{L}_{Q} + (1 - \gamma) \sigma_Q$
\State $\phi^r$ $\gets$ $\overline{\phi^r}$ - $\zeta \nabla \mathcal{L}$ \Comment{Model updates using customized loss}



\EndFor

\Else{ Sever's dataset is considered}
\State Randomly split server's dataset $D^S$ into $m$ sets
\State Each participant $j \in m$ has their own dataset $D_j$ without splitting into support and query sets
\For {Each communication round $r = 1, 2, ..., R$}
\State Participants download global model $\phi^{r-1}$
\For {Each participant $j$ in parallel}
\State Initialize each local model $\phi_j$ with $\phi^{r-1}$
\State $\mathcal{L}_{D_j}(\phi)$ $\gets$ $\frac{1}{|D_j|}$ $\sum_{(x,y) \in D_j}{} \ell(f_\phi(x), y)$
\State $\phi_{j}$ $\gets$ $\phi^{r-1}$ - $\eta \nabla \mathcal{L}_{D_j}(\phi)$ \Comment{Local update using local dataset $D_j$}
\EndFor
\State $\overline{\phi^r}$ $\gets$ $\sum_{j=1}^{m} \mu_j \phi_j$  \Comment{Model aggregation; $\mu_j$ is the relative dataset size}
% \State Server executes updates using split $D^S$

\For {Each split server's dataset $D^S_j$ in parallel, Server}
% \State Initialize each local model $\phi_j$ with $\overline{\phi^r}$
\State $\mathcal{L}_{D^S_j}(\phi)$ $\gets$ $\frac{1}{|D^S_j|}$ $\sum_{(x,y) \in D^S_j}{} \ell(f_\phi(x), y)$ \Comment{Server executes meta--update with split $D^S$}
\EndFor
\State Overall loss on server: $\mathcal{L}_{D^S} = \sum_{j=1}^{m} \mathcal{L}_{D^S_j}(\phi)$; standard deviation of losses: $\sigma_{D^S}$
\State Customized Loss: $\mathcal{L} = \gamma \mathcal{L}_{D^S} + (1 - \gamma) \sigma_{D^S}$
\State $\phi^r$ $\gets$ $\overline{\phi^r}$ - $\zeta \nabla \mathcal{L}$ \Comment{Model updates using customized loss}
\EndFor

\EndIf

\State \textbf{Obtaining a pre-trained model for fine-tuning phase:} $\Phi$ $\gets$ $\phi^R$
\end{algorithmic}
\end{algorithm*}
% \vspace{-\baselineskip} 




\begin{algorithm*}[t]
% \begin{algorithm}
\caption{{\system} Our Pre-training Method (Pre-training Phase in Scenario I)}
\label{alg:alg_pretrain}
\begin{algorithmic}[1]
\State \textbf{Input:} Server dataset $D^S$, Client dataset $D^C$ 
\State Split $D^C$ to $M$ clients based on IID or non-IID distribution, and select $m \in M$ participants.
\State Each participant $j \in m$ partitions their own dataset $D_j$ into support set $S_j$ and query set $Q_j$
\For {Each communication round $r = 1, 2, ..., R$}
\State Participants download global model $\phi^{r-1}$
\For {Each participant $j$ in parallel}
\State Initialize each local model $\phi_j$ with $\phi^{r-1}$
\State $\mathcal{L}_{S_j}(\phi)$ $\gets$ $\frac{1}{|S_j|}$ $\sum_{(x,y) \in S_j}{} \ell(f_\phi(x), y)$
\State $\phi_{j}$ $\gets$ $\phi^{r-1}$ - $\eta \nabla \mathcal{L}_{S_j}(\phi)$ \Comment{Local update using support set $S_j$}
\EndFor
% \State $\overline{\phi^r}$ $\gets$ $\sum_{j=1}^{m} \frac{|S_j|}{|S|} \phi_j$
\State $\overline{\phi^r}$ $\gets$ $\sum_{j=1}^{m} \mu_j \phi_j$ \Comment{Model aggregation; $\mu_j$ is the relative support set size}
\For {Each participant $j$ in parallel}
% \State Initialize each local model $\phi_j$ with $\overline{\phi^r}$
\State Participants download $\overline{\phi^r}$ for initialization and perform meta-updates
\State $\mathcal{L}_{Q_j}(\phi)$ $\gets$ $\frac{1}{|Q_j|}$ $\sum_{(x,y) \in Q_j}{} \ell(f_\phi(x), y)$ \Comment{Local meta-update using query set $Q_j$}
\EndFor
\State Overall meta-loss: $\mathcal{L}_{Q} = \sum_{j=1}^{m} \mathcal{L}_{Q_j}(\phi) $; standard deviation of meta-losses: $\sigma_Q$ 
\State Customized Loss: $\mathcal{L} = \gamma \mathcal{L}_{Q} + (1 - \gamma) \sigma_Q$
\State $\phi^r$ $\gets$ $\overline{\phi^r}$ - $\zeta \nabla \mathcal{L}$ \Comment{Model updates using customized loss}
\EndFor
\State \textbf{Obtaining a pre-trained model for fine-tuning phase:} $\Phi$ $\gets$ $\phi^R$
\end{algorithmic}
\end{algorithm*}
% \vspace{-\baselineskip} 




\begin{algorithm*}[t]
% \begin{algorithm}
\caption{{\system} Our Pre-training Method (Pre-training Phase in Scenario II)}
\label{alg:alg_pretrain}
\begin{algorithmic}[1]
\State \textbf{Input:} Server dataset $D^S$, Client dataset $D^C$ 
\State Split $D^C$ to $M$ clients based on IID or non-IID distribution, and select $m \in M$ participants.
\State Each participant $j \in m$ partitions their own dataset $D_j$ into support set $S_j$ and query set $Q_j$

\State Randomly split server's dataset $D^S$ into $m$ sets
\State Each participant $j \in m$ has their own dataset $D_j$ without splitting into support and query sets
\For {Each communication round $r = 1, 2, ..., R$}
\State Participants download global model $\phi^{r-1}$
\For {Each participant $j$ in parallel}
\State Initialize each local model $\phi_j$ with $\phi^{r-1}$
\State $\mathcal{L}_{D_j}(\phi)$ $\gets$ $\frac{1}{|D_j|}$ $\sum_{(x,y) \in D_j}{} \ell(f_\phi(x), y)$
\State $\phi_{j}$ $\gets$ $\phi^{r-1}$ - $\eta \nabla \mathcal{L}_{D_j}(\phi)$ \Comment{Local update using local dataset $D_j$}
\EndFor
\State $\overline{\phi^r}$ $\gets$ $\sum_{j=1}^{m} \mu_j \phi_j$  \Comment{Model aggregation; $\mu_j$ is the relative dataset size}
% \State Server executes updates using split $D^S$

\For {Each split server's dataset $D^S_j$ in parallel, Server}
% \State Initialize each local model $\phi_j$ with $\overline{\phi^r}$
\State $\mathcal{L}_{D^S_j}(\phi)$ $\gets$ $\frac{1}{|D^S_j|}$ $\sum_{(x,y) \in D^S_j}{} \ell(f_\phi(x), y)$ \Comment{Server executes meta--update with split $D^S$}
\EndFor
\State Overall loss on server: $\mathcal{L}_{D^S} = \sum_{j=1}^{m} \mathcal{L}_{D^S_j}(\phi)$; standard deviation of losses: $\sigma_{D^S}$
\State Customized Loss: $\mathcal{L} = \gamma \mathcal{L}_{D^S} + (1 - \gamma) \sigma_{D^S}$
\State $\phi^r$ $\gets$ $\overline{\phi^r}$ - $\zeta \nabla \mathcal{L}$ \Comment{Model updates using customized loss}
\EndFor

\State \textbf{Obtaining a pre-trained model for fine-tuning phase:} $\Phi$ $\gets$ $\phi^R$
\end{algorithmic}
\end{algorithm*}
% \vspace{-\baselineskip} 

==> Tab/Alg_pretraining_scenario1.tex <==
\begin{algorithm*}[t]
\small
% \begin{algorithm}
\caption{Our Pre-training Method {\system} (Pre-training Phase in {\tt Scenario} I)}
\label{alg:scenario1}
\begin{algorithmic}[1]
\STATE \textbf{Input:} A set of  clients $M$ in the pre-training phase, with each client $i$ holding its pre-training dataset $D^p_i$.
% participate in CoPreFL , each partipant clients each holds dataset $D^P_$
% Client dataset $D^C$ 
% \State Split $D^C$ to $M$ clients based on IID or non-IID distribution, and select $m \in M$ participants.
% \State Each participant $j \in m$ partitions their own dataset $D_j$ into support set $S_j$ and query set $Q_j$
\FOR {Each pre-training round $t = 1, 2, ..., T$} 
\STATE Randomly select a set of clients $m \subset M$  to participate in learning
\STATE Each participant $j \in m$ partitions its own dataset $D^p_j$ into support set $S_j$ and query set $Q_j$
% \State Participants download global model $\phi^{t-1}$
\FOR {Each participant $j$ in parallel}
\STATE Download $\Phi^{t-1}$ from the server 
\FOR{local epoch $e = 1, 2, ..., E$}
% \STATE $\ell^{e}_{S_j}(\Phi^{t}) \gets \frac{1}{|S_j|} \sum_{(x,y)\in S_j} \ell(\Phi^{t-1}(x), y)$ \hfill\Comment{// Compute local support loss at each epoch}
\STATE $\ell^{e}_{S_j}(\Phi^{t}) \gets \frac{1}{|S_j|} \sum_{(x,y)\in S_j} \ell(\Phi^{t,e}_j(x), y)$ \hfill\Comment{// Compute local support loss at each epoch}
\STATE $\Phi^{t,e}_{j}$ $\gets$ $\Phi^{t,e-1}_{j}$ $-$ $\eta \nabla \ell^{e}_{S_j}(\Phi^t)$ \hfill\Comment{// Perform SGD local update using support loss}
\ENDFOR
% \STATE $\mathcal{L}_{S_j}(\Phi^t)$ $\gets$ $\frac{1}{E}$ $\sum_{e = 1}^{E} \ell^{e}_{S_j}(\Phi^t)$ \hfill\Comment{// Compute averaged support loss}
% \STATE $\Phi^t_{j}$ $\gets$ $\Phi^{t-1}$ $-$ $\eta \nabla \mathcal{L}_{S_j}(\Phi^t)$ \hfill\Comment{// Perform SGD local update using averaged support loss $\mathcal{L}_{S_j}$}
\ENDFOR
% \State $\overline{\phi^r}$ $\gets$ $\sum_{j=1}^{m} \frac{|S_j|}{|S|} \phi_j$
% \STATE $\overline{\Phi^t}$ $\gets$ $\sum_{j \in m} \frac{|S_j|}{\sum_{i \in m}|S_i|} \Phi^t_j$ \hfill\Comment{// Model aggregation to construct temporary global model}
\STATE $\overline{\Phi^t}$ $\gets$ $\sum_{j \in m} \frac{|S_j|}{\sum_{i \in m}|S_i|} \Phi^{t,E}_j$ \hfill\Comment{// Model aggregation to construct temporary global model}
\FOR {Each participant $j$ in parallel}
% \State Initialize each local model $\phi_j$ with $\overline{\phi^r}$
\STATE Download $\overline{\Phi^t}$ from the server
\STATE $\mathcal{L}_{Q_j}(\overline{\Phi^t})$ $\gets$ $\frac{1}{|Q_j|}$ $\sum_{(x,y) \in Q_j}{} \ell(\overline{\Phi^t}(x), y)$ \hfill\Comment{// Compute local loss (and gradient) using query set $Q_j$}
\ENDFOR
\STATE Server computes overall meta-loss $\mathcal{L}_{Q}(\overline{\Phi^t})$ and variance across meta-losses $\sigma_Q^2(\overline{\Phi^t})$ according to~\eqref{eq:ourobj}
\STATE $\mathcal{L}_{meta}(\overline{\Phi^t}) = \gamma \mathcal{L}_{Q}(\overline{\Phi^t}) + (1 - \gamma) \sigma_Q^2(\overline{\Phi^t})$  \hfill\Comment{// Customized query meta-loss}
\STATE $\Phi^t$ $\gets$ $\overline{\Phi^t}$ $-$ $\zeta \nabla \mathcal{L}_{meta}(\overline{\Phi^t})$ \hfill\Comment{// Meta-learning model update using customized loss}
\ENDFOR
\STATE \textbf{Output:} A pre-trained model for downstream FL tasks: $\Phi^T$
\end{algorithmic}
\end{algorithm*}
% \vspace{-5mm}
\setlength{\textfloatsep}{7pt}

%\vspace{-\baselineskip} 




==> Tab/C100_sc1_FedProx_qFL.tex <==

 \begin{wraptable}{r}{0.4\textwidth}
 % \begin{table}
\begin{center}
    % \vspace{-5mm}

\scalebox{0.6}{

\begin{tabular}{c||cc||cc}
\hline
% \multirow{2}{c||}{\textbf{Pre-training}(Scenario I)} & \multicolumn{4}{c}{Downstream}\\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {\textbf{Pre-training}} \\ {(Scenario I)}\end{tabular}} & \multicolumn{4}{c}{\textbf{Downstream}: Non-IID FL}\\
\cline{2-5}
 & \multicolumn{2}{c||}{FedProx (\mu = 1)}& \multicolumn{2}{c}{q-FFL (q = 2)}\\
\hline\hline
 {\textbf{Method}} & \textbf{Acc} \uparrow & \textbf{Variance} \downarrow & \textbf{Acc} \uparrow & \textbf{Variance} \downarrow \\
\hline

	
	
		
	
	
	
	
	
	
 {Centralized} & 82.39 & 51.46 & 79.26 & 47.10\\
{FedAvg} & 79.53 & 46.15 & 79.53 & 44.59 \\
{FedMeta} & 81.77 & 63.12 & 79.30 & 39.63\\
{q-FFL} & 83.19 & 52.12 & 81.38 & 37.27 \\
\systemnott & \textbf{84.31} &	\textbf{30.55} & \textbf{82.71} & \textbf{25.39}\\
\hline

\hline

\end{tabular}
}
 \vspace{-2mm}
 \caption{\small Applications of  other FL algorithms during downstream scenarios on CIFAR-100 \yun{replace}.}
%\caption{Comparison using other fairness-aware downstream FL algorithms on CIFAR-100.}
% \vspace{-0.1in}

\label{tb:cfiar_fedprox_qfl}
\end{center}
 % \end{table} 
\end{wraptable} 


==> Tab/main_C100_sc1_pre20_downnoniid.tex <==
\begin{table*}
% \vspace{-8mm}
\small
\begin{center}
\scalebox{0.8}{
\begin{tabular}{c||cccccc}
\hline
{\textbf{Pre-training} (Scenario I)} & \multicolumn{5}{c}{\textbf{Downstream:} Non-IID FedAvg}\\
\hline\hline
 {\textbf{Method}} & \textbf{Acc} \uparrow & \textbf{Variance} \downarrow & \textbf{Worst 10\%} \uparrow& \textbf{Worst 20\%} \uparrow&\textbf{Worst 30\%} \uparrow\\
\hline


{FedAvg} & 78.96 &	64.80 &		62.70 &	67.00 &	69.80\\
{FedMeta} & 82.45 &	48.72 &	68.97 &	72.41 &	74.35\\
 {q-FFL} & 80.01 & 88.92 &		64.39 &	67.48 & 70.30\\
 \systemnott (\gamma = 0.75) & \textbf{83.29} &	\textbf{34.69} &		\textbf{71.58} &	\textbf{73.20} &	\textbf{74.59}\\
\hline
\end{tabular}
}
% \caption{Average performance across 10 non-IID downstream FL tasks, initialized with various FL pre-trained methods using 20 out of 100 distributed participants, on the CIFAR-100 dataset.\yun{revmove m}}
\vspace{-1.5mm}
\caption{\textbf{Scenario I (CIFAR-100):} Average performance across 10 non-IID downstream FL tasks, initialized with various non-IID FL pre-trained models.}
% \vspace{-1.5pc}
\label{tb:main_cfiar_20_noniidfinetune}
\end{center}
% \vspace{-3mm}
\end{table*}


==> Tab/main_tiny_sc1_pre20_downnoniid.tex <==
\begin{table*}
\small
\begin{center}
\scalebox{0.8}{
\begin{tabular}{c||cccccc}
\hline
{\textbf{Pre-training} (Scenario I)} & \multicolumn{5}{c}{\textbf{Downstream:} Non-IID FedAvg}\\
\hline\hline
 {\textbf{Method}} & \textbf{Acc} \uparrow & \textbf{Variance} \downarrow & \textbf{Worst 10\%} \uparrow& \textbf{Worst 20\%} \uparrow&\textbf{Worst 30\%} \uparrow\\
\hline




{FedAvg} & 82.94 &	37.21 &		68.99 &	72.29 &	74.40\\
 {FedMeta} & 81.03 &	37.58 &		69.44 &	71.55 &	72.93\\
 {q-FFL} & 84.11 &	43.96 &		73.87 &	76.05 &	77.37\\
 \systemnott (\gamma = 0.5) & \textbf{85.23} &	\textbf{35.40} &	\textbf{76.77} &	\textbf{78.46} &	\textbf{79.86}\\
\hline
\end{tabular}
}
\vspace{-1.5mm}
\caption{\textbf{Scenario I (Tiny-ImageNet):} Average performance across 10 non-IID downstream FL tasks, initialized with various non-IID FL pre-trained model.}
%\caption{Average performance across 10 non-IID downstream FL tasks, initialized with various FL pre-trained methods in scenario I, on the Tiny-ImageNet dataset.}
% \vspace{-1.5pc}
\label{tb:main_tiny_20_noniidfinetune}
\end{center}
% \vspace{-3.5mm}
\end{table*}


==> aaai_checklist.tex <==
\section{Reproducibility Checklist}

\begin{enumerate}

\item This paper:


\begin{itemize}
  \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA). \textcolor{blue}{Yes}

  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no). \textcolor{blue}{Yes}
  
  \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no). \textcolor{blue}{Yes}
\end{itemize}


\item Does this paper make theoretical contributions? (yes/no) \textcolor{red}{No}

\item Does this paper rely on one or more datasets? (yes/no) \textcolor{blue}{Yes}

\begin{itemize}
  \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA). \textcolor{blue}{Yes}

  \item All novel datasets introduced in this paper are included in a data appendix (yes/partial/no/NA). \textcolor{gray}{NA}
  
  \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
. \textcolor{gray}{NA}

    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) \textcolor{blue}{Yes}

    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) \textcolor{blue}{Yes}

    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) \textcolor{gray}{NA}
\end{itemize}


\item Does this paper include computational experiments? (yes/no) \textcolor{blue}{Yes}


\begin{itemize}
  \item Any code required for pre-processing data is included in the appendix. (yes/partial/no). \textcolor{blue}{Yes}

  \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
 \textcolor{blue}{Yes}
  
  \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) \textcolor{blue}{Yes}

\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) \textcolor{blue}{Yes}

\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) \textcolor{blue}{Yes}

\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) \textcolor{blue}{Yes}

\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) \textcolor{blue}{Yes}

\item This paper states the number of algorithm runs used to compute each reported result. (yes/no)
 \textcolor{blue}{Yes}

  \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)  \textcolor{blue}{Yes}

  \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)  \textcolor{blue}{Yes}

  \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) \textcolor{blue}{Yes}

  \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)
\textcolor{blue}{Yes}


\end{itemize}


\end{enumerate}



